Learning to Generate Cost-to-Go Functions for Efficient Motion Planning

Traditional motion planning is computationally burdensome for practical robots, involving extensive collision checking and considerable iterative propagation of cost values. We present a novel neural network architecture which can directly generate the cost-to-go (c2g) function for a given configuration space and a goal configuration. The output of the network is a continuous function whose gradient in configuration space can be directly used to generate trajectories in motion planning without the need for protracted iterations or extensive collision checking. This higher order function (i.e. a function generating another function) representation lies at the core of our motion planning architecture, c2g-HOF, which can take a workspace as input, and generate the cost-to-go function over the configuration space map (C-map). Simulation results for 2D and 3D environments show that c2g-HOF can be orders of magnitude faster at execution time than methods which explore the configuration space during execution. We also present an implementation of c2g-HOF which generates trajectories for robot manipulators directly from an overhead image of the workspace.

==> bkup/old_intro.tex <==
Motion planning algorithm requires to generate collision-free trajectories rapidly. Search-based planning approaches such as A* and D* can generate an optimal path \cite{bonet2001planning,maximARA,stentz1995focussed}, but these search-based planning algorithms require discretization of space; thus they are computationally intractable in high-dimensional space. Sampling based planning approaches such as Probabilistic RoadMap (PRM) and Randomly exploring Random Trees (RRT) are popular due to their simplicity and flexibility \cite{lavalle2001randomized,kavraki1996probabilistic}, but their performance depends on sampling methods or local steering algorithms. Although there are many variation of sampling based planning approaches to overcome these limitations, it is very hard to overcome a critical disadvantage that the performance is significantly degraded in complicated configuration spaces\cite{karaman2011anytime,bekris2003multiple,urmson2003approaches,jaillet2010sampling,gammell2014informed}.

To address problems of traditional planning approaches, we suggest a learning approach with deep neural networks which estimates cost-to-go values in the configuration space from a given workspace information. There are several learning approaches based on deep neural networks \cite{ichter2018learning,qureshi2018motion,molinalearning,zhang2018learning,zhang2019auto}. \cite{ichter2018learning} suggests Conditional variational autoencoder (CVAE) for sampling policies, and \cite{qureshi2018motion} learns motion planning networks encoding the workspace into latent feature space. However these approaches require successful trajectory exemplars or pre-defined features in workspace for conditioning variables. Therefore, it is hard to adept to a changing conditions. In addition, Since the networks is not able to generate a trajectory alone, they suggest hybird algorithms combining the network with a traditional planning algorithm. On the other hand, our suggested deep neural network can estimate cost-to-go values in C-space from workspace without heavy computation, and it help a planner to generate trajectory quickly without mapping between workspace and C-space using inverse and forward kinematics. we use Higher Order Functions (HOF) Network to represent the cost-to-go of C-space while HOF network is used for 3D shape reconstruction in previous work \cite {mitchell2019higher,wang2020geodesic}.

The core contributions of the paper include a novel network for cost-to-go estimation of configuration space with High Order Functions (HOF) networks; 2) Cmap network to estimate collision probability of configuration samples instantly; 3) HOF network encoding the collision probablity into the weights and biases of the secondary decoder network; 4) the decoder network with small parameters predicting cost values of sample configurations. Since the network is small for cost estimation, it can generate trajectory efficiently, and it can adapt to chaning environment by updating the weights and biases of decoder network via encoder network. This paper evaluates the performance of HOF planning network in simulation and verifies the network with a physical robot system.
     

==> old_insight.tex <==
%\volkan{JInwook, this paragraph can move to discussion}
 Our results indicate that a neural network can be trained to output a continuous cost-to-go function over a given workspace. The same network can be adapted to various setting simply by changing the encoder architecture:  We used the exact same  c2g-network except for input sample dimension for 2DoF and 3DoF cases. It shows that HOF-network can learn any c2g-network appropriately based on appropriate input data and architecture.
 
For the network training, sampling strategies are important. Sparse sampling makes hard the network converge, and dense uniform sampling takes long time for training. We samples around collision boundary for meaningful samples and mixed negative samples from collision regions. 

To prevent the network is biased to easy cases or too complicated, we make good dataset distribution over complexity of workspace. Since the network is trained with well distributed dataset, we can translate trained network performance onto the real system well. In addition, although the network is trained with discretized cost-to-go from Dijkstra, the c2g function by the c2g-network is continous function; thus it is useful for real-system compared to Dijkstra planner.

 Since HOF network encodes \cmap{} into the weights and biases of the c2g-network from a given workspace and it is unnecessary to update c2g-network parameters, we can use the only c2g-network for cost-to-go estimation for planning in a given workspace. Since the c2g-network has only 256 parameters, the planning is very fast. In addition, when the environment is changed, the C-map network and HOF-network quickly update the weights and biases of c2g-network without heavy computation. Therefore, \ours{} is efficient for planning in various environment.
 
 Finally, we show that end-to-end learning is possible with this network architecture from workspace to plan in C-space. We can generate c2g function in various dimensions and cases according to HOF network architecture designs. 

==> to-do.tex <==
1. abstract [Volkan] -v1 complete
2. captions esp. figure 1   -capitalization /ours
3. add one paragraph in Section 2 describing the network incl. loss function and training data generation
3.5 new histograms [jw]
4. finish up section 5 [Volkan]

send the paper to Helen


spell check

suppl. material
- details of how we randomly generate workspace

\ours. 
\ours{} is great.

here is a reference~\cite{xxx}.
daksljdaklsjadl 
skjasd [10] dasdlakjsasdkj


histogram

2-link manipulator
3-dof manipulator

C-map network (or cmap network)
HOF network  (or HOF-network)
c2g-network



Notes from meeting with Dan:

- Mention Sergey Levine's value iteration network
they do it over the whole map
https://arxiv.org/abs/1602.02867
